A Game Theoretical Analysis of Localization Security in Wireless Sensor Networks with Adversaries

Wireless Sensor Networks (WSN) support data collection and distributed data processing by means of very small sensing devices that are easy to tamper and cloning: therefore classical security solutions based on access control and strong authentication are difficult to deploy. In this paper we look at the problem of assessing security of node localization. In particular, we analyze the scenario in which Verifiable Multilateration (VM) is used to localize nodes and a malicious node (i.e., the adversary) try to masquerade as non-malicious. We resort to non-cooperative game theory and we model this scenario as a two-player game. We analyze the optimal players' strategy and we show that the VM is indeed a proper mechanism to reduce fake positions.

==> extensive.tex <==
\section{Analysis as an extensive game}
\label{sec:extensive}

==> scenario.tex <==
\section{Reference Scenario}
\label{sec:reference-scenario}

We consider a dense network composed of nodes $n$, where $n \in N$
and a base station $b$ in which all the collected data sink.
 The network architecture  is shown in Fig. \ref{fig:topology}. It is
assumed a many-to-one convergent traffic going hop-by-hop in the
upstream direction from many sensor nodes to the sink node
\cite{baronti:07}. Each sensor node can deal two types of traffic:
source and transit.Therefore, each sensor node can act as a source
of data and/or as forwarding element.
 We consider two subsets of $N$:
\begin{itemize}
\item $S$, composed by nodes $s_i, 0 < i \leq |S|$ which perform
  sensing functions;


\item $V$, composed by nodes $v_i, 0 < i \leq |V|$ which work as
  verifiers in the secure localization protocol.
\end{itemize}

$N = S  \cup V$, however $V$ may overlap $S$ (in principle every
node whose position can be taken for granted might be used as a
verifier). In particular, as starting point we consider an
application domain in which there are only three verifiers which
directly communicate (at one hop distance) with  a node whose
position is unknown.



\begin{figure}[htbp]
\centering
\includegraphics[width=6.5 cm]{topology}
\caption{Network topology.} \label{fig:topology}
\end{figure}

Each $s_i$ node senses a given type of data (\textit{e.g.,}
temperature, pressure, brightness, position and so on). Each node
(sensing, and verifier) directly communicates with its closer
neighbours (at one hop distance).



%%% Local Variables:
%%% mode: latex
%%% ispell-local-dictionary: "english"
%%% TeX-master: "globecom10"
%%% End:

